The free-fermionic $C^{(1)}_2$ loop model, double dimers and Kashaev's recurrence

We study a two-color loop model known as the $C^{(1)}_2$ loop model. We define a free-fermionic regime for this model, and show that under this assumption it can be transformed into a double dimer model. We then compute its free energy on periodic planar graphs. We also study the star-triangle relation or Yang-Baxter equations of this model, and show that after a proper parametrization they can be summed up into a single relation known as Kashaev's relation. This is enough to identify the solution of Kashaev's relation as the partition function of a $C^{(1)}_2$ loop model with some boundary conditions, thus solving an open question of Kenyon and Pemantle about the combinatorics of Kashaev's relation.

==> tikz/face2.tex <==
\begin{tikzpicture}[scale=0.12]
\draw (-2,0) -- (0,-1) -- (2,0) -- (0,1) -- cycle;
  \draw (-2,0) node [left] {$\Scale[0.8]{x}$};
  \draw (2,0) node [right] {$\Scale[0.8]{y}$};
  \draw (0,1) node [above] {$\Scale[0.8]{u}$};
  \draw (0,-1) node [below] {$\Scale[0.8]{v}$};
\end{tikzpicture}


==> tikz/l2.tex <==
\begin{tikzpicture}[scale=0.3]
  \draw [gray, dashed, fill opacity=0.7,fill=white!90!black] (-2,0) -- (0,-1.3) -- (2,0) -- (0,1.3) -- cycle;
  \draw [ultra thick, color=red, rounded corners=6pt] (-1.3,1) -- (0,0) -- (-1.3,-1);
  \draw [ultra thick, color=blue, rounded corners=6pt] (1.3,1) -- (0,0) -- (1.3,-1);
  \draw (-1.2,0.9) node [] {$2$};
  \draw (-1.2,-0.9) node [] {$2$};
\end{tikzpicture}


==> tikz/l3.tex <==
\begin{tikzpicture}[scale=0.3]
  \draw [gray, dashed, fill opacity=0.7,fill=white!90!black] (-2,0) -- (0,-1.3) -- (2,0) -- (0,1.3) -- cycle;
  \draw [ultra thick, color=blue, rounded corners=6pt] (-1.3,1) -- (0,0) -- (-1.3,-1);
  \draw [ultra thick, color=blue, rounded corners=6pt] (1.3,1) -- (0,0) -- (1.3,-1);
\end{tikzpicture}


==> tikz/l3a.tex <==
\begin{tikzpicture}[scale=0.3]
  \draw [gray, dashed, fill opacity=0.7,fill=white!90!black] (-2,0) -- (0,-1.3) -- (2,0) -- (0,1.3) -- cycle;
  \draw [ultra thick, color=blue, rounded corners=6pt] (-1.3,1) -- (0,0) -- (1.3,1) ;
  \draw [ultra thick, color=blue, rounded corners=6pt] (-1.3,-1) -- (0,0) -- (1.3,-1);
\end{tikzpicture}


==> tikz/l5.tex <==
\begin{tikzpicture}[scale=0.3]
  \draw [gray, dashed, fill opacity=0.7,fill=white!90!black] (-2,0) -- (0,-1.3) -- (2,0) -- (0,1.3) -- cycle;
  \draw [ultra thick, color=red] (-1.3,1) -- (0,0) -- (1.3,-1);
  \draw [ultra thick, color=blue] (1.3,1) -- (0,0) -- (-1.3,-1);
  \draw (-1.2,0.9) node [] {$2$};
  \draw (1.2,-0.9) node [] {$0$};
\end{tikzpicture}


==> tikz/l6.tex <==
\begin{tikzpicture}[scale=0.3]
  \draw [gray, dashed, fill opacity=0.7,fill=white!90!black] (-2,0) -- (0,-1.3) -- (2,0) -- (0,1.3) -- cycle;
  \draw [ultra thick, color=red, rounded corners=6pt] (-1.3,1) -- (0,0) -- (-1.3,-1);
  \draw [ultra thick, color=blue, rounded corners=6pt] (1.3,1) -- (0,0) -- (1.3,-1);
  \draw (-1.2,0.9) node [] {$0$};
  \draw (-1.2,-0.9) node [] {$0$};
\end{tikzpicture}


==> tikz/orient.tex <==
%% Creator: Inkscape inkscape 0.92.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'orient.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{88.6711725bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.6745821)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{orient.pdf}}%
  \end{picture}%
\endgroup%


==> tikz/qloop.tex <==
%% Creator: Inkscape inkscape 0.92+devel, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'loop.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{48.58291054bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.04614993)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{loop.pdf}}%
  \end{picture}%
\endgroup%

